The Non-Uniform k-Center Problem

In this paper, we introduce and study the Non-Uniform k-Center problem (NUkC). Given a finite metric space $(X,d)$ and a collection of balls of radii $\{r_1\geq \cdots \ge r_k\}$, the NUkC problem is to find a placement of their centers on the metric space and find the minimum dilation $\alpha$, such that the union of balls of radius $\alpha\cdot r_i$ around the $i$th center covers all the points in $X$. This problem naturally arises as a min-max vehicle routing problem with fleets of different speeds. The NUkC problem generalizes the classic $k$-center problem when all the $k$ radii are the same (which can be assumed to be $1$ after scaling). It also generalizes the $k$-center with outliers (kCwO) problem when there are $k$ balls of radius $1$ and $\ell$ balls of radius $0$. There are $2$-approximation and $3$-approximation algorithms known for these problems respectively; the former is best possible unless P=NP and the latter remains unimproved for 15 years. We first observe that no $O(1)$-approximation is to the optimal dilation is possible unless P=NP, implying that the NUkC problem is more non-trivial than the above two problems. Our main algorithmic result is an $(O(1),O(1))$-bi-criteria approximation result: we give an $O(1)$-approximation to the optimal dilation, however, we may open $\Theta(1)$ centers of each radii. Our techniques also allow us to prove a simple (uni-criteria), optimal $2$-approximation to the kCwO problem improving upon the long-standing $3$-factor. Our main technical contribution is a connection between the NUkC problem and the so-called firefighter problems on trees which have been studied recently in the TCS community.

==> kcwo.tex <==
\newcommand{\parent}{\ensuremath{{\sf parent}}\xspace}
\subsection{LP-Aware Tree Embedding for two types of radii}
As a warm-up to our general algorithm, let us consider the case when there are only two types of radius. Indeed, let $(M,k_1,k_2,r_1,r_2)$ be an instance of \nukc where the goal is to find placement of $k_1$ balls of radius $r_1$ and $k_2$ balls of radius $r_2$ such that they together cover all the points in the metric space $M = (X,d)$. As mentioned earlier, a useful special case to understand would be the one where $r_1 =r$ and $r_2 = 0$, in which case the problem becomes the \kcwo problem.

To best understand our approach for the general \nukc problem, let us see how the algorithm in~\cite{CKMN01} solves the \kcwo problem, and comprehend the difficulties in extending it for multiple radius types. Indeed, the algorithm in~\cite{CKMN01} is a greedy-like procedure which we now sketch: at each step, they greedily pick the ball of radius $r$ which contains the maximum number of uncovered points, and include the $3r$ ball as a cluster. They claim that after $k$ iterations, we would have at most $z$ points uncovered. Indeed, the reason is that at each stage, since we pick the densest ball, we can argue that we are not picking a ball all of whose points OPT declared as outliers. Therefore, by expanding the ball to radius $3r$, we can conclude that we would fully cover one new OPT cluster entirely at each step.

But notice that the above approach crucially uses the fact that points are either outliers, or are covered by a ball of radius $r$, and is hard to generalize to even $3$ types of radii. Therefore, to circumvent the aforementioned difficulties, we appeal to an LP-based approach, where we can hopefully infer which clients are better off covered by clusters of which radius type. As a welcome side-effect, we also obtain improved algorithms for the \kcwo problem, which we now describe as warm-up to our general reduction.

 We now discuss a natural LP for the \kcwo problem. For each input point $p$, there are two indicator variables $y_{p}$ and $z_{p}$. The variable $y_p$ is the indicator variable for whether $p$ is the center of a cluster of size $r$, and the variable $z_p$ decides if $p$ is treated as an outlier or not.


\begin{alignat}{2}
\label{lp1:1} \sum_{q: d(p,q) \leq r}{y_q}  +   z_p & \geq & \, \, 1 \\
\label{lp1:2}   \sum_{p}{y_p} & \leq& k \\
\label{lp1:3}   \sum_{p}{z_p} & \leq &\ell
\end{alignat}
%\textbf{$LP_{kCWO}$} &\\

Let $(y^*,z^*)$ be an optimal solution to the above LP. We will use this solution to create a collection of stars where the set of all leaves correspond exactly to the points in the metric space, and the roots correspond to a set of potential centers we may open clusters around. We will ensure that the distance between any leaf and the root of the corresponding star is at most $2r$, so a cluster of radius $2r$ around the root vertex would cover all the leaves. 

We would also assign a fractional solution $(\widetilde{y},\widetilde{z})$ where the $\widetilde{y}$ variables will be assigned to the roots, and the $\widetilde{z}$ vertices will be assigned to the leaves such that for any leaf $p$ with corresponding root $q$, we have $\widetilde{z}_p + \widetilde{y}_{q} \geq 1$, and moreover, the total $\widetilde{y}$ fractional value would be at most $k$ and the total $\widetilde{z}$ value, at most $\ell$. This fractional solution is then a feasible solution to the LP relaxation for the problem of picking $k$ roots such that all but $\ell$ leaves are covered.

Next we will show that the above LP on these stars is in fact integral. Finally, we show how to map a solution on the stars back to one on the original metric space, precisely by choosing clusters of radius $2r$ around the root vertices and leaving all uncovered outliers as leaves. 


\begin{algorithm}
\caption{Tree-Embedding for \kcwo}
\label{alg:kcwo}
\label{alg:createTree}
\begin{algorithmic}
% \KwData{$U=\{u_1,u_2,...u_n\}$, $(y,z)$ and $k$}
% \KwResult{Tree $T$}
\STATE Mark all points $p \in P$ as 'uncovered'
\WHILE{There exists an uncovered point $p \in P$}
\STATE Choose the uncovered point $p$ with minimum coverage $\cov(p,0)$ (call it a winner)
\STATE Let $N_p$ denote the set of all uncovered points $q$ such that $d(p,q) \leq 2r$
\STATE Create a new root $w$ corresponding to $p$, define $\psi(w) = p$ to identify $w$ with $p$ 
\STATE Form a star connecting $w$ to the set of leaves $N_p \cup \{p\}$
\STATE Mark $p$ and all $q \in N_p$ as covered
\STATE Set $\widetilde{y}_{w} = \cov(p,1)$
\ENDWHILE
\end{algorithmic}
\end{algorithm}
\medskip


For the below claims, let $\parent(p)$ denote the root vertex to which the leaf $p$ is connected to. The variables $\widetilde{y}$ for the roots are as defined in the algorithm above, and we simply define $\widetilde{z}_p = z^*_p$ for all the leaves $p \in P$.
\begin{claim} \label{cl:newlp}
The fractional solution $(\widetilde{y},\widetilde{z})$ is a feasible solution for the following constraints: (a) $ \widetilde{z}_p + \widetilde{y}_{\parent(p)} \geq 1 \, \, \forall p \in P$, (b) $ \sum_{w} \widetilde{y}_w \leq k $, and (c) $\sum_{p} \widetilde{z}_p \leq \ell$.

\end{claim}

\begin{proof}
We show that the fractional solution satisfies these constraints one by one. Consider $p \in P$, and suppose $p$ is connected to a root vertex $w$ which corresponds to point $q$ (i.e., $\psi(w) = q$). Then, by the way we have created the stars, we know that that $\cov(q,0) \leq \cov(p,0)$. Moreover, since $(x^*,y^*)$ is feasible for the \nukc LP, we have from eq~\eqref{lp1:1} that $\cov(q,1) \geq 1 - \cov(q,0) \geq 1 - \cov(p,0)$. This combined with our definition of $\widetilde{z}_{p}$ and $\widetilde{y}_{w}$ then suffices to show constraints (a) for all $p$.

As for the outlier constraint (c), they are trivially satisfied because $\sum_{p} \widetilde{z}_{w} = \sum_{p} z^*_p \leq \ell$. Finally, for constraint (b), note have that for any pair of root vertices $w$ and $w'$ of different stars, the balls $B(\psi(w),r)$ and $B(\psi(w'),r)$ are disjoint in the original metric space. Therefore, $\sum_{w} \widetilde{y}_w  = \sum_{w} \cov(\psi(w),1) = \sum_{w} \sum_{q \in B(\psi(w) ,r)} y^*_q \leq k$.
\end{proof}

\begin{claim}
We can efficiently round the fractional solution $(\widetilde{y},\widetilde{z})$ to a feasible integral solution satisfying the constraints (a), (b) and (c) above in~\Cref{cl:newlp}.
\end{claim}

\begin{proof}
If there exists no root $w$ such that $0 < \widetilde{y}_w <1$, then it is easy to see that $(\widetilde{y},\widetilde{z})$ itself is an integral solution. Otherwise, there exists at least two root nodes $w$ and $w'$ with fractional values assigned to them. Now, without loss of generality, let us assume that $|C(w)| \geq |C(w')|$, where $C(w)$ is the set of children of $w$. Now for some small constant $0< \epsilon <1$, we do the following:
$\widetilde{y}_w := \widetilde{y}_{w} + \epsilon$, $\widetilde{y}_{w} := \widetilde{y}_{w'} - \epsilon$, $ \forall c \in C(w),\; y_c := y_c - \epsilon$, and $\forall c \in C(w'),\; y_c := y_c + \epsilon$.

Note that the sum of $\widetilde{y}$ values remains the same, and so the constraint (b) is still satisfied. Also observe that the sum of $\widetilde{z}$ values for nodes on level $0$ either remains the same or decreases, because $|C(w) \geq |C(w')|$. Hence we do not violate the outlier constraint (c) as well. Finally, the constraints~\eqref{lp1:1} are also satisfied because the sum $\widetilde{y_w} + \widetilde{y_c}$ is preserved for any root $w$ and child $c$.

We can repeat this procedure as long as there exists a pair in $T$ that has fractional values in $\widetilde{y}$. Once we have exhausted all such pairs, we know that all nodes at level $1$ in $T$ have integral $\widetilde{y}$ values. This in return ensures that all the leaf nodes in $T$ also have integral $y$ values, by constraint (a). 
\end{proof}

Finally, we now prove that we can recover a $2$-approximate solution to the \kcwo problem on the original metric space. Indeed, if the integral solution from~\Cref{cl:round} opens a root vertex $w$, we open a cluster of radius $2r$ around a node $\psi(w)$. And likewise, if the integral solution does not pick a root vertex $w$, we then make all its children outliers. It is easy to see, using the fact that the distance between the original points associated with any root and child is at most $2r$ in the original metric space, that this results in the desired $2$-approximation for the original \kcwo instance.

